Program Analysis with Local Policy Iteration

We present a new algorithm for deriving numerical invariants that combines the precision of max-policy iteration with the flexibility and scalability of conventional Kleene iterations. It is defined in the Configurable Program Analysis (CPA) framework, thus allowing inter-analysis communication. It uses adjustable-block encoding in order to traverse loop-free program sections, possibly containing branching, without introducing extra abstraction. Our technique operates over any template linear constraint domain, including the interval and octagon domains; templates can also be derived from the program source. The implementation is evaluated on a set of benchmarks from the Software Verification Competition (SV-Comp). It competes favorably with state-of-the-art analyzers.

==> diagrams/abstract_semantics_concavity.tex <==
\begin{tikzpicture}[auto, transform shape, scale=1.4]
    \tikzset{font=\tiny}

    % Axis.
    %\draw[help lines,step=.2, gray, very thin] (-2,-2) grid (7,4);
    %\draw[help lines,line width=.6pt,step=1] (-2,-2) grid (7,4);
    %\foreach \x in {-2,-1,0,1,2,3,4,5,6,7}
    %\node[anchor=north] at (\x,-2) {\x};
    %\foreach \y in {-2,-1,0,1,2,3,4}
    %\node[anchor=east] at (-2,\y) {\y};
    \coordinate (initial) at (0, 0);
    \coordinate (top) at (1.5, 3);

    \draw[->, >=stealth] (-1.6, 0) -> node[very near end] {$t$} (4,0);
    \draw[->, >=stealth] ($ -0.4*(top)$) -> node[very near end] {$t'$} (top);


    % Polyhedra.
    \draw (2, 0.1) -> (1, 1) coordinate (highest) -> (-1, 0.5) coordinate (second)
        -> (-1.5, -0.6) coordinate (third)
        node[red, anchor=south west, xshift=0.2cm, yshift=0.2cm, font=\tiny]
            {$G(x)$} -> (2, 0.1) coordinate (last);

    \fill[red] (highest) circle (1pt)
        node[font=\tiny, anchor=south west, black, xshift=-0.4cm]{$\max{t' x}
            \mbox{ s.t. } G x \leq 0$};
    \coordinate (projection) at ($(initial)!(highest)!(top)$);
    \coordinate (rightmost) at ($(projection)!5!(highest)$);

    \fill (projection) circle (1pt);

    % Abstract semantics
    \foreach \x in {0, 0.2, ..., 1}
        \fill[red] ($(highest)!\x!(rightmost)$) circle (1pt);

    \foreach \x in {0, 0.20, ..., 1}
        \fill[red] ($(highest)!\x!(second)$) circle (1pt);

    \foreach \x in {0, 0.33, ..., 1}
        \fill[red] ($(second)!\x!(third)$) circle (1pt);

    \draw[gray, very thin, red, dashed] (rightmost)
        node[anchor=south west,font=\tiny]{$f^{\sharp}(d)$} -> (highest) -> (second) -> (third);

    \fill[red, opacity=0.2] (highest) -> (second) -> (third) -> (last);

    % Moving constraint
    \draw[blue] (rightmost) ++ (0, -2) coordinate(r_b)
        node[font=\tiny, anchor=south east]{$t x \leq d$} -- node[anchor=north west]{$d$} ++(0, 3.8);

    \fill[blue, opacity=0.1] (r_b) rectangle (-2, 2);

\end{tikzpicture}


==> diagrams/extra_transitions_example.tex <==
% Example of extra transitions avoided by dynamic path focusing.
\begin{tikzpicture}[auto, scale=1, transform shape]
    \node (loop_a) [program_node] {$1$};
    \node (loop_b) [program_node, right=2 of loop_a] {$2$};
    \node (loop_c) [program_node, right=2 of loop_b] {$3$};
    \node (merge) [program_node, below=2 of loop_b] {Merge};

    \path[transition] (loop_a) edge[loop above] node {} (loop_a);
    \path[transition] (loop_b) edge[loop above] node {} (loop_b);
    \path[transition] (loop_c) edge[loop above] node {} (loop_c);

    \draw [transition] (loop_a.south) to (merge.north);
    \draw [transition] (loop_b.south) to (merge.north);
    \draw [transition] (loop_c.south) to (merge.north);
\end{tikzpicture}


==> diagrams/self_map.tex <==
% Fixpoints of the monotone concave function.
\begin{tikzpicture}[auto, scale=0.9, transform shape]
    % x = y
    \draw[name path=straight, thick](0, 0) -- node[font=\tiny, very near end, anchor=west]{$y=x$}(3.7, 3.7);

    % coordinate lines.
    \draw[->] (0, 0) -> node[anchor=north, very near end]{$x$} (4, 0);
    \draw[->] (0, 0) -> node[anchor=east, very near end]{$y$} (0, 4);

    % Concave function.
    \draw[name path=concave, blue, very thick, dashed](0.3, -0.3)  .. controls (0.9, 2.5) and (2.5, 3.1) ..
        node[anchor=south, font=\tiny, text width=1cm, xshift=-0.5cm, yshift=-0.1cm]
        {$y=f(x)$}
    (3.6, 3);

    \fill [blue, name intersections={of=straight and concave}]
        (intersection-1) circle (1pt)
            node[opacity=1, anchor=west, font=\tiny] {$f_1 = f(f_1)$}
        (intersection-2) circle (1pt)
            node[opacity=1, anchor=south east, font=\tiny] {$f_2 = f(f_2)$};


    \fill[black] (1, 1) coordinate (initial) circle (1pt)
            node[opacity=1, anchor=north west, font=\tiny] {$x_0$};

    % Fixpoint iterations.
    \path[name path=vertical] (initial) -- +(0, 2);
    \fill[black, name intersections={of=vertical and concave}]
        (intersection-1) coordinate(f_1) circle (1pt) 
        ;

    \path[name path=horizontal_1] (f_1) -- +(2, 0);
    \fill[black, name intersections={of=horizontal_1 and straight}]
        (intersection-1) coordinate(f_2) circle(1pt)
        node[font=\tiny, anchor=west]{$f(x_0)$};

    \path[name path=vertical_2] (f_2) -- +(0, 2);
    \fill[black, name intersections={of=vertical_2 and concave}]
        (intersection-1) coordinate(f_3) circle(1pt);

    \path[name path=horizontal_2] (f_3) -- +(2, 0);
    \fill[black, name intersections={of=horizontal_2 and straight}]
        (intersection-1) coordinate(f_4) circle(1pt)
        node[font=\tiny, anchor=west]{$f(f(x_0))$};

    \path[name path=vertical_3] (f_4) -- +(0, 2);
    \fill[black, name intersections={of=vertical_3 and concave}]
        (intersection-1) coordinate(f_5) circle(1pt);

    \path[name path=horizontal_3] (f_5) -- +(2, 0);
    \fill[black, name intersections={of=horizontal_3 and straight}]
        (intersection-1) coordinate(f_6) circle(1pt)
        node[font=\tiny, anchor=west, text width=2cm]
        {$f(f(f(x_0)))$};


    \draw[->, thin, shorten >=2pt,>=stealth] (initial) -> (f_1);
    \draw[->, thin, shorten >=2pt,>=stealth] (f_1) -> (f_2);
    \draw[->, thin, shorten >=2pt,>=stealth] (f_2) -> (f_3);
    \draw[->, thin, shorten >=2pt,>=stealth] (f_3) -> (f_4);
    \draw[->, thin, shorten >=2pt,>=stealth] (f_4) -> (f_5);
    \draw[->, thin, shorten >=2pt,>=stealth] (f_5) -> (f_6);

\end{tikzpicture}


==> diagrams/very_simple_cfg.tex <==
\begin{tikzpicture}[auto, scale=1, transform shape]
    \node(entry) [] {};
    \node (a) [program_node, below=0.6 of entry] {A};
    \draw [transition, loop below] (a) to node {$i \leq 10 \land i' = i+1$} (a);
    \draw [transition] (entry) to node {$i' = 0$} (a);
\end{tikzpicture}

